Best-Effort Communication Improves Performance and Scales Robustly on Conventional Hardware

Here, we test the performance and scalability of fully-asynchronous, best-effort communication on existing, commercially-available HPC hardware. A first set of experiments tested whether best-effort communication strategies can benefit performance compared to the traditional perfect communication model. At high CPU counts, best-effort communication improved both the number of computational steps executed per unit time and the solution quality achieved within a fixed-duration run window. Under the best-effort model, characterizing the distribution of quality of service across processing components and over time is critical to understanding the actual computation being performed. Additionally, a complete picture of scalability under the best-effort model requires analysis of how such quality of service fares at scale. To answer these questions, we designed and measured a suite of quality of service metrics: simulation update period, message latency, message delivery failure rate, and message delivery coagulation. Under a lower communication-intensivity benchmark parameterization, we found that median values for all quality of service metrics were stable when scaling from 64 to 256 process. Under maximal communication intensivity, we found only minor -- and, in most cases, nil -- degradation in median quality of service. In an additional set of experiments, we tested the effect of an apparently faulty compute node on performance and quality of service. Despite extreme quality of service degradation among that node and its clique, median performance and quality of service remained stable.

==> Makefile <==
# get the basename of the containing directory
# this will be used to name othe output document
BUILD_DIR := $(shell basename $(abspath $(dir $(lastword $(MAKEFILE_LIST)))))

all: ${BUILD_DIR}-draft.pdf

view:
	atom ${BUILD_DIR}.pdf

${BUILD_DIR}.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR} \
    -pdflatex="pdflatex -interaction=nonstopmode" main.tex

${BUILD_DIR}-draft.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR}-draft \
    -pdflatex="pdflatex -interaction=nonstopmode" draft.tex

fresh: cleaner all

clean:
	rm -f ${BUILD_DIR}.pdf
	rm -f ${BUILD_DIR}-draft.pdf

sview:
	xdg-open ${BUILD_DIR}-draft.pdf 2>/dev/null

cleaner:
	latexmk -CA
	# remove auxillary files, excepting .tex and .bib files
	find . -type f -name ${BUILD_DIR}"*" ! -name '*.tex' ! -name '*.bib' -delete


==> draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> submodule/2021-gecco-conduit/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> submodule/2021-gecco-conduit/fig/conduit.tex <==
   \begin{figure}[thpb]
      \centering
      \includegraphics[width=0.8\linewidth]{img/conduit}
      \caption{Schematic of Conduit's \texttt{Inlet} and \texttt{Outlet} object scheme.
      Intra-thread, inter-thread, or inter-process communication behavior is performed by an underlying \texttt{Duct} object.
      The underlying communication mechanism used is transparent to the end-user.
      }
      \label{fig:conduit}
   \end{figure}

==> submodule/2021-gecco-conduit/tex/abstract.tex <==
\begin{abstract}
% Developing software to effectively take advantage of growth in parallel and distributed processing capacity poses significant challenges.
% Best-effort computing models have been proposed as a strategy to overcome challenges around harnessing high performance computing at extreme scale.
% These models relax synchronization and hardware reliability requirements, accepting nondeterminism in exchange for efficiency.
% This trade-off, inherent to best-effort computing, is often compatible with nature-inspired computing methods.
% Although many programming languages and frameworks aim to facilitate software development for high performance applications, existing tools do not directly provide a prepackaged best-effort interface.
% The Conduit C++ Library aims to provide a convenient interface for best-effort inter-thread and inter-process communication.
% Here, we describe the motivation, objectives, design, and implementation of the library.
% Benchmarks on a communication-intensive graph coloring problem and a compute-intensive digital evolution simulation, show that Conduit's best-effort model can improve scaling efficiency and solution quality, particularly in a distributed, multi-node context.

% Conduit will be useful facilitated efficient, scalable parallel and distributed implementations of natural computing algorithms.

Developing software to effectively take advantage of growth in parallel and distributed processing capacity poses significant challenges.
Traditional programming techniques allow a user to assume that execution, message passing, and memory are always kept synchronized.
However, maintaining this consistency becomes increasingly costly at scale. 
One proposed strategy is ``best-effort computing'', which relaxes synchronization and hardware reliability requirements, accepting nondeterminism in exchange for efficiency.
Although many programming languages and frameworks aim to facilitate software development for high performance applications, existing tools do not directly provide a prepackaged best-effort interface.
The Conduit C++ Library aims to provide such an interface for convenient implementation of software that uses best-effort inter-thread and inter-process communication.
Here, we describe the motivation, objectives, design, and implementation of the library.
Benchmarks on a communication-intensive graph coloring problem and a compute-intensive digital evolution simulation show that Conduit's best-effort model can improve scaling efficiency and solution quality, particularly in a distributed, multi-node context.
%% Conduit will be useful facilitated efficient, scalable parallel and distributed implementations of natural computing algorithms. (this is why you care as a GP person)

\end{abstract}




==> submodule/2021-gecco-conduit/tex/acknowledgements.tex <==
\begin{acks}
\footnotesize
This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.

\end{acks}

==> submodule/2021-gecco-conduit/tex/conclusion.tex <==
\section{Conclusion}

Benchmarks show that best-effort communication through Conduit enables significantly better computational performance under high thread and process counts.
We also demonstrated how, in the case of the graph coloring benchmark, best-effort communication can help achieve tangibly better solution quality within a fixed time constraint, as well.  
We observed the greatest relative speedup under distributed communciation-heavy workloads --- about $7.8\times$ on the graph coloring benchmark.
Distributing the computation-heavy digital evolution benchmark workload across independent nodes yielded the strongest scaling of our benchmarks, achieving at 64 processes 92\% the update-rate of single-process execution. 

In future work, we plan to further characterize the performance of the Conduit's best-effort model with respect to the digital evolution simulation, looking directly at quality of service metrics such as message latency and frequency of dropped messages.
We are also eager to investigate how Conduit's best-effort communication model scales on much larger process counts, perhaps on the order of hundreds or thousands of cores.

Development of the Conduit library stemmed from a practical need for an abstract, prepackaged interface to support our digital evolution research.
We hope that making this library available to the community can reduce domain expertise and programmability barriers to taking advantage of the best-effort communication model to efficiently leverage burgeoning parallel and distributed computing power. 

==> submodule/2021-gecco-conduit/tex/design.tex <==
\section{Library Design}

\input{fig/conduit.tex}

The Conduit C++ Library aims to compliment the parallel and distributed programming ecosystem by providing an abstracted best-effort interface to application programmers.
Under Conduit's interface, more recent messages may preempt existing ones, messages may be dropped under backlog conditions, and read operations may opt to view the most recently received message in lieu of waiting for an expected message.

Conduit represents communication in terms of a paired \texttt{Inlet}, which accepts messages, and \texttt{Outlet}, which dispenses messages.
An \texttt{Inlet} and \texttt{Outlet} may exchange messages via an intra-thread, inter-thread, or inter-process communication procedure, depending on the runtime state of an underlying \texttt{Duct} object.
Figure \ref{fig:conduit} provides a schematic overview.
The implementation of intra-thread, inter-thread, and inter-process communication procedures may be configured at compile-time.
Conduit provides a library of intra-thread, inter-thread, and inter-process implementations to choose from and allows end-users to build their own.

The \texttt{Inlet} provides a non-blocking \texttt{TryPut()} method, which attempts to queue a message for its corresponding \texttt{Outlet} but may drop it under backlog conditions, as well as a \texttt{Put()} method, which block under backlog conditions until buffer space is available to queue the message is available.
The \texttt{Outlet} provides a \texttt{TryStep()} and \texttt{Jump()} methods to load the next or latest message, respectively.
If no new messages are available, the last-received message will be accessed.
The \texttt{Outlet} also provides a \texttt{Step()} method, which will block until a new message is received.
At run time, \texttt{Duct}s can be created or modified to perform intrathread, interthread, or interprocess communication. 

In addition to this granular connection-level interface, Conduit provides a network-level interface where the user defines their computation in terms of a directed graph.
In this network topology, nodes represent simulation elements and edges represent communication channels.
The library will assign nodes in that topology to available threads across available processes and automatically instantiate appropriate conduits.
Individual threads of execution can then launch and freely process computational updates on their assigned nodes while receiving messages from nodes assigned to other processes as they become available.
Conduit provides several pre-defined standard topologies and node-assignment algorithms.
However, users can also opt to use the NetworkX graph library \cite{hagberg2008exploring} to generate arbitrary topologies and the METIS software package \cite{gupta1997fast} to automatically balance expected load across available threads and processes while minimizing inter-process and inter-thread communication.

Defining program logic in terms of atomic, inter-communicating simulation elements provides significant programmability advantages.
Such code can be written in terms of interactions between intuitive domain-specific objects (e.g., digital organisms that interact with one another, subpopulations with migration, etc.), while leaving the task of mapping onto hardware resources to automatic management by the underlying framework.
However, a naive implementation of this approach would entail significant inefficiency, particularly with inter-process communication which has a large overhead.
Imagine, for example, a processes dispatching independent MPI calls for each communication channel between another process and the thousands of atomic simulation elements it holds.
Conduit addresses this issue by providing duct implementations that automatically consolidate messages between processes into single MPI calls.
These implementations support a ``pooling'' mechanism, in which a consolidated MPI call is dispatched once each constituent \texttt{Inlet} has received a single message, and a ``aggregation'' mechanism, in which arbitrary numbers of messages can be contributed from each \texttt{Inlet}.

Conduit is made freely available under a MIT License as a header-only C++17 software package at \url{https://github.com/mmore500/conduit}.
Conduit was built using the cereal C++11 Library for serialization \cite{voorhies2017cereal} and the Empirical C++ Library \cite{charles_ofria_2019_2575607}.


==> submodule/2021-gecco-conduit/tex/implementation.tex <==
\section{ Implementation }

Conduit's implementation has been developed around the following principles.

\begin{itemize}
    \item \textbf{overdecomposition}: Conduit provides a uniform API for intra-thread, inter-thread, and inter-process communication between agents.
    \item \textbf{testability}: Interchangeablility of inter-thread and inter-process communication for intra-thread communication makes software more readily unit-testable.
    \item \textbf{don't use what you don't want}: Multi-thread execution may be performed without MPI runtime.
    \item \textbf{don't pay for what you don't use}: Intra-thread, inter-thread, and inter-process communication are explicitly handled by separate, optimized implementations. 
    \item \textbf{modularity}: Different intra-thread, inter-thread, or inter-process implementations can be trivially interchanged for rapid prototyping and tuning.
    \item \textbf{flexibility}: Communication primitives may trivially rearranged to form arbitrary network structures. 
    \item \textbf{extensibility}: Users may provide communication implementations or network topologies.
    \item \textbf{lightweight}: The core components of Conduit are built as a header-only library.
    \item \textbf{portability}: Conduit is built using MPI and C++17 standards.
    \item \textbf{interoperability}: Conduit is compatible with other multithread and MPI code.
    \item \textbf{simplicity}: Conduit manages resource initialization and lifetime automatically.
    % \item \textbf{intuitiveness}: TODO object-oriented model with a simple API and an intuitive real-world analogy.
\end{itemize}

Source code is hosted on GitHub at \url{https://github.com/mmore500/conduit}, made freely available under a MIT License.
Documentation is hosted on ReadTheDocs at \url{https://conduit.fyi}.
A containerized build environment for Conduit is hosted on DockerHub at \url{https://hub.docker.com/r/mmore500/conduit}.

==> submodule/2021-gecco-conduit/tex/introduction.tex <==
\section{Introduction}

The parallel and distributed processing capacity of high-performance computing clusters continues to grow rapidly and enable profound scientific and industrial innovations \cite{gagliardi2019international}.    
Hardware advances afford great opportunity, but also pose a serious challenge: developing approaches to effectively harness it.
As HPC systems scale, deterministic algorithms depending on global synchronization become increasingly costly \cite{gropp2013programming,dongarra2014applied}.

Best-effort computing, where data dependencies are relaxed to reduce synchronization \cite{chakradhar2010best}, can improve scalability \cite{meng2009best}.
Evolutionary algorithms typically perform perform a search or optimization with many acceptable results using pseudo-stochastic methods.
Algorithms with these properties can often tolerate significant perturbations, including relaxation of synchronization requirements in the underlying algorithm.
For example, island model genetic algorithms have been shown to perform well with asynchronous migration \cite{izzo2009parallel}.
While not the focus of this paper, the original interest that motivated development of the Conduit library stems from work exploring open-ended evolution.
Researchers in this domain study long-term dynamics of evolutionary systems in order to understand factors that affect these systems' potential to generate ongoing novelty \cite{taylor2016open}.
Some recent evidence suggests that the generative potential of systems devised to study open-ended evolution is --- at least in part --- meaningfully constrained by available compute resources \cite{channon2019maximum}.
Such observations raise the question of how to design parallel and distributed open-ended evolution systems.

The concept of indefinite scalability was developed to describe constraints distributed systems would face at the asymptote of technological (and even physical) constraints.
Indefinite scalability theory posits that such systems would necessitate
\begin{itemize}
    \item asynchronous operation,
    \item decentralized networking,
    \item interchangeable components (i.e., no global identifiers),
    \item and graceful degradation under hardware failure \cite{ackley2011pursue}.
\end{itemize}
Although bespoke experimental hardware such as Illuminato X machina has been developed to demonstrate aspects of the indefinite scalability paradigm \cite{ackley2011homeostatic}, practical contemporary work scaling up evolving systems necessitates working with commercially-available hardware.
However, existing distributed computing frameworks for contemporary high-performance computing hardware do not explicitly expose a convenient best-effort interface.
In our current work, we focus on asynchronous operation and decentralization.
We leave system robustness and resistance to hardware degradation to future work.

The Message Passing Interface (MPI) standard \cite{gropp1996high} represents the mainstay for high-performance computing applications.
This standard exposes communication primitives directly to the end user.
MPI's nonblocking communication primitives, in particular, are sufficient to program distributed computations with relaxed synchronization requirements.
Although its explicit, imperative nature enables precise control over execution, it also poses significant expense in terms of programability.
This cost manifests in terms of programmer productivity, domain knowledge requirements, software quality, and difficulty tuning for performance due to program brittleness \cite{gu2019comparative, tang2014mpi}.

In response to programmability concerns, many frameworks have arisen to offer useful parallel and distributed programming abstractions.
Task-based frameworks such as Charm++ \cite{kale1993charm++}, Legion \cite{bauer2012legion}, Cilk \cite{blumofe1996cilk}, and Threading Building Blocks (TBB) \cite{reinders2007intel} describe the dependency relationships among computational tasks and associated data and relies on an associated runtime to automatically schedule and manage execution.
These frameworks assume a deterministic relationship between tasks.
In a similar vein, programming languages and extensions like Unified Parallel C (UPC) \cite{el2006upc} and Chapel \cite{chamberlain2007parallel} rely on programmers to direct execution, but equips them with powerful abstractions, such as global shared memory.
However, Chapel's memory model explicitly forbids data races and UPC ultimately relies on a barrier model for data transfer.

==> submodule/2021-gecco-conduit/tex/methods.tex <==
\section{Methods}

We performed two benchmarks to compare the performance of Conduit's best-effort approach to a traditional synchronous model.
We tested our benchmarks across both a multithread, shared-memory context and a distributed, multinode context.
In each hardware context, we assessed performance on two algorithmic contexts: a communication-intensive distributed graph coloring problem (Section \ref{sec:graph_coloring_benchmark}) and a compute-intensive digital evolution simulation (Section \ref{sec:digital_evolution_benchmark}).
The latter benchmark --- presented in Section \ref{sec:digital_evolution_benchmark} --- grew out of the original work developing the Conduit library to support large-scale experimental systems to study open-ended evolution.
The former benchmark --- presented in Section \ref{sec:graph_coloring_benchmark} --- complements the first by providing a clear definition of solution quality.
Metrics to define solution quality in the open-ended digital evolution context remain a topic of active research.

\subsection{ Graph Coloring Benchmark } \label{sec:graph_coloring_benchmark}

The graph coloring benchmark employs a graph coloring algorithm designed for distributed WLAN channel selection \cite{leith2012wlan}.
In this algorithm, nodes begin by randomly choosing a color.
Each computational update, nodes test for any neighbor with the same color.
If and only if a conflicting neighbor is detected, nodes randomly select another color.
The probability of selecting each possible color is stored in array associated with each node.
Before selecting a new color, the stored probability of selecting the current (conflicting) color is decreased by a multiplicative factor $b$.
We used $b=0.1$, as suggested by Leith et al.
Likewise, the stored probability of selecting all others is increased by a multiplicative factor.
Regardless of whether their color changed, nodes transmit their current color to their neighbor.

Our benchmarks focus on weak scalability, using a fixed problem size of 2048 graph nodes per thread or process.
These nodes were arranged in a two-dimensional grid topology where each node had three possible colors and four neighbors.
We implement the algorithm with a single Conduit communication layer carrying graph color as an unsigned integer.
We used Conduit's built-in pooling feature to consolidate color information into a single MPI message between pairs of communicating processes each update.
We performed five replicates, each with a five second simulation runtime.
Solution error was measured as the number of graph color conflicts remaining at the end of the benchmark.

\subsection{ Digital Evolution Benchmark } \label{sec:digital_evolution_benchmark}

The digital evolution benchmark runs the DISHTINY (DIStributed Hierarchical Transitions in Individuality) artificial life framework.
This system is designed to study major transitions in evolution, events where lower-level organisms unite to form a self-replicating entity.
The evolution of multicellularity and eusociality exemplify such transitions.
Previous work with DISHTINY has explored methods for selecting traits characteristic of multicellularity such as reproductive division of labor, resource sharing within kin groups, resource investment in offspring, and adaptive apoptosis \cite{moreno2019toward}.

DISHTINY simulates a fixed-size toroidal grid populated by digital cells.
Cells can sense attributes of their immediate neighbors, can communicate with those neighbors through arbitrary message passing, and can interact with neighboring cells cooperatively through resource sharing or competitively through antagonistic competition to spawn daughter cells into limited space.
This cell behavior is controlled by SignalGP event-driven linear genetic programs \cite{lalejini2018evolving}.
Full details of the DISHTINY simulation are available in \cite{moreno2021exploring}.

We use Conduit-based messaging channels to manage all interactions between neighboring cells.
During a computational update, each cell advances its internal state and pushes information about its current state to neighbor cells.
Several independent messaging layers handle disparate aspects of cell-cell interaction, including
\begin{itemize}
  \item Cell spawn messages, which contain arbitrary-length genomes (seeded at 100 12-byte instructions with a hard cap of 1000 instructions). These are handled every 16 updates and use Conduit's built-in aggregation support for inter-process transfer.
  \item Resource transfer messages, consisting of a 4-byte float value. These are handled every update and use Conduit's built-in pooling support for inter-process transfer.
  \item Cell-cell communication messages, consisting of arbitrarily many 20-byte packets dispatched by genetic program execution. These are handled every 16 updates and use Conduit's built-in aggregation support for inter-process transfer.
  \item Environmental state messages, consisting of a 216-byte struct of data. These are handled every 8 updates and use conduit's built-in pooling support for inter-process transfer.
  \item Multicellular kin-group size detection messages, consisting of a 16-byte bitstring. These are handled every update and use Conduit's built-in pooling support for inter-process transfer.
\end{itemize}

Implementing all cell-cell interaction via Conduit-based messaging channels allows the simulation to be parallelized down to the granularity, potentially, of individual cells.
However, in practice, for this benchmarking we assign 3600 cells to each thread or process.
Because all cell-cell interactions occur via Conduit-based messaging channels, logically-neighboring cells can interact fully whether or not they are located on the same thread or process (albeit with potential irregularities due to best-effort limitations).
An alternate approach to evolving large populations might be an island model, where Conduit-based messaging channels would be used solely to exchange genomes between otherwise independent populations \cite{bennett1999building}.
However, we chose to instead parallelize DISHTINY as a unified spatial realm in order to enable parent-offspring interaction and leave the door open for future work with multicells that exceed the scope of an individual thread or process.

\subsection{Asynchronicity Modes} \label{sec:asynchronicity_modes}

\input{fig/asynchronicity_modes.tex}

For both benchmarks, we compared performance across a spectrum of synchronization setting, which we term ``asynchronicity modes'' (Table \ref{tab:asynchronicity_modes}).
Asynchronicity mode 0 represents traditional fully-synchronous methodology.
Under this treatment, full barrier synchronization was performed between each computational update.
Asynchronicity mode 3 represents fully asynchronous methodology.
Under this treatment, individual threads or processes performed computational updates freely, incorporating input from other threads or processes on a fully best-effort basis.

During early development of the library, we discovered that unprocessed messages building up faster than they could be processed --- even if they were being skipped over to only get the latest message --- could degrade quality of service or even cause runtime instability.
We opted for MPI communication primitives that could consume many backlogged messages per call and increased buffer size to address these issues, but remained interested in the possibility of partial synchronization to clear potential message backlogs.
So, we included two partially-synchronized treatments: asynchronicity modes 1 and 2.

In asynchronicity mode 1, threads and processes alternated between performing computational updates for a fixed-time duration and executing a global barrier synchronization.
For the graph coloring benchmark, work was performed in 10ms chunks.
For the digital evolution benchmark, which is more computationally intensive, work was performed in 100ms chunks.
In asynchronicity mode 2, threads and processes executed global barrier synchronizations at predetermined time points.
In both experiments, global barrier synchronization occurred on each time a second of epoch time elapsed.

Finally, asynchronicity mode 4 disables all inter-thread and inter-process communication, including barrier synchronization.
We included this mode to isolate the impact on performance of communication between threads and processes from other factors potentially affecting performance, such as cache crowding.
In this run mode for the graph coloring benchmark, all calls to put messages into or pull messages out of ducts between processes or threads were skipped (except after the benchmark concluded, when assessing solution quality).
Because of its larger footprint, incorporating logic into the digital evolution simulation to disable all inter-thread and inter-process messaging was impractical.
Instead, we launched multiple instances of the simulation as fully-independent processes and measured performance of each.

\subsection{Code, Data, and Reproducibility}

Benchmarking experiments were performed on [redacted for double-blind review]'s High Performance Computing Center, a cluster of hundreds of heterogeneous x86 nodes linked with InfiniBand interconnects.
For multithread experiments, benchmarks for each thread count were collected from the same node.
For multiprocess experiments, each processes was assigned to a distinct node in order to ensure results were representative of performance in a distributed context.
All multiprocess benchmarks recorded from the same collection of nodes.
Hostnames are recorded for each benchmark data point.
For an exact accounting of hardware architectures used, these hostnames can be crossreferenced with a table included with the data that summarizes the cluster's node configurations.

Code for the distributed graph coloring benchmark is available at \url{https://github.com/mmore500/conduit} under \\ \texttt{demos/channel\_selection}.
Code for the digital evolution simulation benchmark is available at \url{https://github.com/mmore500/dishtiny}.
Exact versions of software used are recorded with each benchmark data point.
Data is available via the Open Science Framework at \url{https://osf.io/7jkgp/} \cite{foster2017open}.
An in-browser notebook for all reported statistics and data visualizations and is available via Binder at \url{https://mybinder.org/v2/gh/mmore500/conduit/binder?filepath=binder%2Fdate%3D2021%2Bproject%3D7jkgp} \citep{jupyter2018binder}.


==> submodule/2021-gecco-conduit/tex/results.tex <==
\section{Results and Discussion}

\subsection{Multithread Benchmarks}

\input{fig/multithread_benchmarks.tex}

Figure \ref{fig:multithread_graph_coloring_update_rate} presents per-cpu algorithm update rate for the graph coloring benchmark at 1, 4, 16, and 64 threads.
Update rate performance decreased with increasing multithreading across all asynchronicity modes.
This performance degradation was rather severe --- per-cpu update rate decreased by 61\% between 1 and 4 threads and by about another 75\% between 4 and 64 threads.
Surprisingly, this issue appears largely unrelated to inter-thread communication, as it was also observed in asynchronicity mode 4, where all interthread communication is disabled.
Perhaps per-cpu update rate degradation under threading was induced by strain on a limited system resource like memory cache or access to the system clock (which was used to control run timing).
This unexpectedly severe phenomenon merits further investigation to fully in future work with this benchmark.

Nevertheless, we were able to observe significantly better performance of best-effort asynchronicity modes 1, 2, and 3 at high thread counts. 
At 64 threads, these run modes significantly outperformed the fully-synchronized mode 0 ($p < 0.05$, non-overlapping 95\% confidence intervals).
Likewise, as shown in Figure \ref{fig:multithread_graph_coloring_solution_quality}, best-effort asynchronicity modes were able to deliver significantly better graph coloring solutions within the allotted compute time than the fully-synchronized mode 0 ($p < 0.05$, non-overlapping 95\% confidence intervals).

Figure \ref{fig:multithread_digital_evolution_update_rate} shows per-cpu algorithm update rate for the digital evolution benchmark at 1, 4, 16, and 64 threads.
Similarly to the graph coloring benchmark, update rate performance decreased with increasing multithreading across all asynchronicity modes --- including mode 4, which eschews inter-thread communication.
Even without communication between threads, with 64 threads each thread performed updates at only 61\% the rate of a lone thread.
At 64 threads, best-effort asynchronicity modes 1, 2, and 3 exhibit about 43\% the update-rate performance of a lone thread.
Although best-effort inter-thread communication only exhibits half the update-rate performance of completely decoupled execution at 64 threads, this update-rate performance is roughly $2.1\times$ that of the fully-synchronous mode 0.
Indeed, best-effort modes significantly outperform the fully-synchronous mode on the digital evolution benchmark at both 16 and 64 threads ($p < 0.05$, non-overlapping 95\% confidence intervals).

\subsection{Multiprocess Benchmarks}

\input{fig/multiprocess_benchmarks.tex}

Figure \ref{fig:multiprocess_graph_coloring_update_rate} shows per-cpu algorithm update rate for the graph coloring benchmark at 1, 4, 16, and 64 processes.
Unlike the multithreaded benchmark, multiprocess graph coloring exhibits consistent update-rate performance across process counts under asynchronicity mode 4, where inter-thread communication is disabled.
This matches the expectation that, indeed, with comparable hardware a single process should exhibit the same mean performance as any number of completely decoupled processes.
At 64 processes, best-effort asynchronicity mode 3 exhibits about 63\% the update-rate performance of single-process execution. 
This represents about an $7.8\times$ speedup compared to fully-synchronous mode 0.
Indeed, best-effort mode 3 enables significantly better per-cpu update rates at 4, 16, and 64 processes ($p < 0.05$, non-overlapping 95\% confidence intervals).

Likewise, shown in Figure \ref{fig:multiprocess_graph_coloring_solution_quality}, best-effort asynchronicity mode 3 yields significantly better graph-coloring results within the allotted time at 4, 16, and 64 processes ($p < 0.05$, non-overlapping 95\% confidence intervals).
Interestingly, partial-synchronization modes 1 and 2 exhibited highly inconsistent solution quality performance at 16 and 64 process count benchmarks.
Fixed-timepoint barrier sync (mode 2) had particularly poor performance performance at 64 processes (note the log-scale axis).
We suspect this was caused by a race condition where workers would assign sync points to different fixed points different based on slightly different startup times (i.e., process 0 syncs at seconds 0, 1, 2... while process 1 syncs at seconds 1, 2, 3..).

Figure \ref{fig:multiprocess_digital_evolution_update_rate} presents per-cpu algorithm update rate for the digital evolution benchmark at 1, 4, 16, and 64 processes.
Relative performance fares well at high process counts under this relatively computation-heavy workload, with 64-process fully best-effort simulation exhibiting about 92\% the update rate of single-process simulation.
This represents a $2.1\times$ speedup compared to the fully-synchronous run mode 0.
Best-effort significantly mode 3 outperforms the per-cpu update rate of fully-synchronous mode 0 at process counts 16 and 64 ($p < 0.05$, non-overlapping 95\% confidence intervals).


==> submodule/conduit-binder/Dockerfile <==
# Pull base image.
FROM ubuntu:bionic-20180125@sha256:d6f6cc62b6bed64387d84ca227b76b9cc45049b0d0aefee0deec21ed19a300bf

COPY . /opt/conduit/

SHELL ["/bin/bash", "-c"]

# Define default working directory.
WORKDIR /opt/conduit

# Prevent interactive time zone config.
# adapted from https://askubuntu.com/a/1013396
ENV DEBIAN_FRONTEND=noninteractive

# adapted from https://users.open-mpi.narkive.com/tEPxZF0B/ompi-users-how-to-get-rid-of-openmpi-warning-unable-to-find-any-relevant-network-interfaces
# see also https://github.com/open-mpi/ompi-www/issues/161#issue-390004007
RUN \
  mkdir -p "/root/.openmpi" \
    && \
  mkdir -p "/home/user/.openmpi" \
    && \
  echo "btl_base_warn_component_unused = 0" >> /etc/openmpi-mca-params.conf \
    && \
  echo "btl_base_warn_component_unused = 0" >> /root/.openmpi/mca-params.conf \
    && \
  echo "btl_base_warn_component_unused = 0" >> /home/user/.openmpi/mca-params.conf \
    && \
  echo "configured system-wide openmpi mca parameters"

RUN \
  echo 'Acquire::http::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::ftp::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::Retries "100";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo "buffed apt-get resiliency"

RUN \
  find /etc/apt -type f -name '*.list' -exec sed -i 's/\(^deb.*-backports.*\)/#\1/; s/\(^deb.*-updates.*\)/#\1/; s/\(^deb.*-proposed.*\)/#\1/; s/\(^deb.*-security.*\)/#\1/' {} + \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "removed -backports, -updates, -proposed, -security repositories"

RUN \
  apt-get update -qq \
    && \
  apt-get install -y --allow-downgrades --no-install-recommends \
    build-essential \
    ca-certificates \
    cmake \
    curl \
    doxygen \
    emacs \
    fonts-liberation \
    gconf-service \
    gdb \
    gpg-agent \
    gzip \
    hdf5-helpers \
    hdf5-tools \
    htop \
    libappindicator1 \
    libasound2 \
    libatk1.0-0 \
    libc6 \
    libcairo2 \
    libcups2 \
    libcurl4 \
    libcurl4-openssl-dev \
    libdbus-1-3 \
    libexpat1 \
    libfontconfig1 \
    libgconf-2-4 \
    libgdk-pixbuf2.0-0 \
    libglib2.0-0 \
    libgtk-3-0 \
    libhdf5-100 \
    libhdf5-cpp-100 \
    libhdf5-dev \
    libhdf5-doc \
    libhdf5-mpi-dev \
    libhdf5-mpich-100 \
    libhdf5-mpich-dev \
    libhdf5-openmpi-100 \
    libhdf5-openmpi-dev \
    libhdf5-serial-dev \
    libmpich-dev \
    libmpich12 \
    libnspr4 \
    libnss3 \
    libopenmpi-dev \
    libopenmpi2 \
    libpango-1.0-0 \
    libpangocairo-1.0-0 \
    libpthread-stubs0-dev \
    libstdc++-7-dev \
    libstdc++6=8-20180414-1ubuntu2 \
    libx11-6 \
    libx11-xcb1 \
    libxcb1 \
    libxcomposite1 \
    libxcursor1 \
    libxdamage1 \
    libxext6 \
    libxfixes3 \
    libxi6 \
    libxrandr2 \
    libxrender1 \
    libxss1 \
    libxtst6 \
    locales \
    lsb-release \
    man \
    mpich \
    multitail \
    nano \
    ninja-build \
    nodejs \
    npm \
    openmpi-bin \
    openmpi-common \
    openmpi-doc \
    openssh-server \
    python-dev \
    python-h5py \
    python-pip \
    python-setuptools \
    python-sphinx \
    python-virtualenv \
    python-wheel \
    python3-dev \
    python3-h5py \
    python3-pip \
    python3-setuptools \
    python3-sphinx \
    python3-virtualenv \
    python3-wheel \
    rsync \
    slurm-client \
    software-properties-common \
    tar \
    unzip \
    vim \
    wget \
    xdg-utils \
    && \
  add-apt-repository ppa:git-core/ppa -y \
    && \
  apt-get update -qq \
    && \
  apt-get install -y --no-install-recommends git \
    && \
  apt-get clean \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "installed fundamentals"

# adapted in part from https://askubuntu.com/a/916451
RUN \
  apt-get update -qq \
    && \
  rm /etc/apt/apt.conf.d/docker-gzip-indexes \
    && \
  apt-get purge apt-show-versions \
    && \
  rm /var/lib/apt/lists/*lz4 \
    && \
  apt-get -o Acquire::GzipIndexes=false update \
    && \
  add-apt-repository -y ppa:ubuntu-toolchain-r/test \
    && \
  wget -O - https://apt.llvm.org/llvm-snapshot.gpg.key | apt-key add - \
    && \
  apt-add-repository "deb https://apt.llvm.org/xenial/ llvm-toolchain-xenial-7 main" \
    && \
  add-apt-repository -y ppa:ubuntu-toolchain-r/test \
    && \
  apt-get update -qq \
    && \
  apt-get clean \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "configured packaging system"

RUN \
  apt-get update -qq \
    && \
  apt-get install -qq \
    libclang-7-dev=1:7.1.0~svn353565-1~exp1~20190408084827.60 \
    llvm-7=1:7.1.0~svn353565-1~exp1~20190408084827.60 \
    llvm-7-dev=1:7.1.0~svn353565-1~exp1~20190408084827.60 \
    clang-7=1:7.1.0~svn353565-1~exp1~20190408084827.60 \
    g++-9=9.4.0-1ubuntu1~18.04 \
    && \
  apt-get clean \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "installed llvm-7 dependencies"

# magic from https://github.com/puppeteer/puppeteer/issues/3451#issuecomment-523961368
RUN echo 'kernel.unprivileged_userns_clone=1' > /etc/sysctl.d/userns.conf

RUN \
  pip3 install  --timeout 60 --retries 100 -r /opt/conduit/third-party/requirements.txt \
    && \
  pip3 install  --timeout 60 --retries 100 -r /opt/conduit/docs/requirements.txt \
    && \
  echo "installed Python packages"

RUN \
  update-alternatives --install /usr/bin/g++ g++ /usr/bin/g++-9 90 \
    && \
  update-alternatives --install /usr/bin/clang++ clang++ /usr/bin/clang++-7 90 \
    && \
  update-alternatives --install /usr/bin/llvm-config llvm-config /usr/bin/llvm-config-7 90 \
    && \
  update-alternatives --install /usr/bin/llvm-profdata llvm-profdata /usr/bin/llvm-profdata-7 90 \
    && \
  update-alternatives --install /usr/bin/llvm-cov llvm-cov /usr/bin/llvm-cov-7 90 \
    && \
  npm install -g n@6.7.0 \
    && \
  n 12.18.2 \
    && \
  export python="/usr/bin/python" \
    && \
  npm install source-map@0.7.3 \
    && \
  echo "finalized dependency versions"

RUN \
  npm install -g jsonlint@1.6.3 \
    && \
  echo "installed npm dependencies"

RUN \
  cd third-party \
    && \
  ./install_dependencies.sh \
    && \
  echo "installed third party dependencies"

# set up locale
# adapted from https://stackoverflow.com/a/55077451
RUN \
  locale-gen en_US.UTF-8 \
    && \
  echo "generated en_US.UTF-8 locale"

# Set enviroment variables
# Use mimalloc override within the container.
ENV LD_PRELOAD=/usr/local/lib/mimalloc-1.6/libmimalloc.so
ENV LC_ALL=C.UTF-8
ENV LANG=C.UTF-8

RUN \
  git remote set-url origin https://github.com/mmore500/conduit.git \
    && \
  echo "switched to https origin remote url"

# Perform any further action as an unprivileged user.
# adapted from https://stackoverflow.com/a/27703359
# and https://superuser.com/a/235398
RUN \
  useradd --create-home --shell /bin/bash user \
    && \
  groupadd group \
    && \
  gpasswd -a user group \
    && \
  chgrp --recursive user /opt \
    && \
  chmod --recursive g+rwx /opt \
    && \
  chmod --recursive g+rwx /home/user \
    && \
  chown -R user /home/user/ \
    && \
  echo "user added and granted permissions to /opt and /home/user"

RUN \
  mkdir /context/ \
    && \
  chown user:user /context/ \
    && \
  mkdir /__w/ \
    && \
  chown user:user /__w/ \
    && \
  echo "/context/ /__w/ directories set up, user granted permissions"

USER user

CMD ["bash"]


==> submodule/conduit-binder/Makefile <==
SHELL := /bin/bash

# Project-specific settings
PROJECT := conduit
EMP_DIR := third-party/Empirical/include/emp

# Flags to use regardless of compiler
CFLAGS_all := -pipe -Wall -Wno-unused-function -std=c++17 -Iinclude/ -fopenmp

# Native compiler information
CFLAGS_nat := -O3 -DNDEBUG -O3 -flto -march=native $(CFLAGS_all)
CFLAGS_nat_debug := -g $(CFLAGS_all)
UIT_MPICXX ?= mpicxx
UIT_MPIEXEC ?= mpiexec

# Emscripten compiler information
CXX_web := emcc
OFLAGS_web_all := -s "EXTRA_EXPORTED_RUNTIME_METHODS=['ccall', 'cwrap']" -s TOTAL_MEMORY=67108864 --js-library $(EMP_DIR)/web/library_emp.js -s EXPORTED_FUNCTIONS="['_main', '_empCppCallback', '_empDoCppCallback']" -s DISABLE_EXCEPTION_CATCHING=1 -s NO_EXIT_RUNTIME=1 #--embed-file configs
OFLAGS_web := -Oz -DNDEBUG
OFLAGS_web_debug := -g4 -Oz -Wno-dollar-in-identifier-extension

CFLAGS_web := $(CFLAGS_all) $(OFLAGS_web) $(OFLAGS_web_all)
CFLAGS_web_debug := $(CFLAGS_all) $(OFLAGS_web_debug) $(OFLAGS_web_all)


default: $(PROJECT)
native: $(PROJECT)
web: $(PROJECT).js documentation-coverage-badge.json version-badge.json doto-badge.json

omp: CFLAGS_nat := $(CFLAGS_nat) -fopenmp
omp: $(PROJECT)

debug: CFLAGS_nat := $(CFLAGS_nat_debug)
debug: $(PROJECT)

debug-web: CFLAGS_web := $(CFLAGS_web_debug)
debug-web: $(PROJECT).js

web-debug: debug-web

$(PROJECT): source/native/$(PROJECT).cpp
	$(UIT_MPICXX) $(CFLAGS_nat) source/native/$(PROJECT).cpp -lstdc++fs -lbenchmark -lmetis -lpthread -o $(PROJECT)
	@echo To build the web version use: make web

$(PROJECT).js: source/web/$(PROJECT)-web.cpp
	source third-party/emsdk/emsdk_env.sh; \
	$(CXX_web) $(CFLAGS_web) source/web/$(PROJECT)-web.cpp -o web/$(PROJECT).js

serve:
	python3 -m http.server

install-coverage-dependencies:
	git submodule init && git submodule update \
		&& cd third-party/force-cover && make

cov: install-coverage-dependencies
	cd tests && make cov

documentation-coverage:
	cd docs && make coverage

documentation-coverage-badge.json: documentation-coverage
	python3 ci/parse_documentation_coverage.py docs/_build/doc-coverage.json > web/documentation-coverage-badge.json

version-badge.json:
	python3 ci/parse_version.py .bumpversion.cfg > web/version-badge.json

doto-badge.json:
	python3 ci/parse_dotos.py $$(./ci/grep_dotos.sh) > web/doto-badge.json

clean:
	rm -f $(PROJECT) web/$(PROJECT).js web/*.js.map web/*.js.map *~ source/*.o web/*.wasm web/*.wast
	rm -rf coverage_include
	cd docs && make clean
	cd demos && make clean
	cd macrobenchmarks && make clean
	cd microbenchmarks && make clean
	cd tests && make clean

docs:
	cd docs && make html

demos:
	cd demos && make

macrobenchmark:
	cd macrobenchmarks && make bench

microbenchmark:
	cd microbenchmarks && make bench

benchmark: macrobenchmark microbenchmark

test-readme-snippets:
	python3 ci/test_readme_snippets.py

test-source: debug debug-web
	$(UIT_MPIEXEC) -n 1 ./conduit | grep -q '>>> end <<<' && echo 'matched!' || exit 1
	npm install
	echo "const puppeteer = require('puppeteer'); var express = require('express'); var app = express(); app.use(express.static('web')); app.listen(3000); express.static.mime.types['wasm'] = 'application/wasm'; function sleep(millis) { return new Promise(resolve => setTimeout(resolve, millis)); } async function run() { const browser = await puppeteer.launch(); const page = await browser.newPage(); await page.goto('http://localhost:3000/conduit.html'); await sleep(1000); const html = await page.content(); console.log(html); browser.close(); process.exit(0); } run();" | node | tr -d '\n' | grep -q "Hello, browser!" && echo "matched!" || exit 1
	echo "const puppeteer = require('puppeteer'); var express = require('express'); var app = express(); app.use(express.static('web')); app.listen(3000); express.static.mime.types['wasm'] = 'application/wasm'; function sleep(millis) { return new Promise(resolve => setTimeout(resolve, millis)); } async function run() { const browser = await puppeteer.launch(); const page = await browser.newPage(); page.on('console', msg => console.log(msg.text())); await page.goto('http://localhost:3000/conduit.html'); await sleep(1000); await page.content(); browser.close(); process.exit(0); } run();" | node | grep -q "Hello, console!" && echo "matched!"|| exit 1

test:
	test $TRAVIS && mkdir -p "~/.openmpi/" && touch "~/.openmpi/mca-params.conf" && grep -qxF 'btl_base_warn_component_used = 0' ~/.openmpi/mca-params.conf || echo 'btl_base_warn_component_used = 0' >> ~/.openmpi/mca-params.conf
	cd tests && make

test-opt:
	test $TRAVIS && mkdir -p "~/.openmpi/" && touch "~/.openmpi/mca-params.conf" && grep -qxF 'btl_base_warn_component_used = 0' ~/.openmpi/mca-params.conf || echo 'btl_base_warn_component_used = 0' >> ~/.openmpi/mca-params.conf
	cd tests && make opt

test-fulldebug:
	test $TRAVIS && mkdir -p "~/.openmpi/" && touch "~/.openmpi/mca-params.conf" && grep -qxF 'btl_base_warn_component_used = 0' ~/.openmpi/mca-params.conf || echo 'btl_base_warn_component_used = 0' >> ~/.openmpi/mca-params.conf
	cd tests && make fulldebug

test-all: test test-opt test-fulldebug

.PHONY: \
	benchmark \
	clean \
	cov \
	demos \
	docs \
	install-coverage-dependencies \
	native \
	macrobenchmark \
	microbenchmark \
	serve \
	test \
	tests \
	web \


# Debugging information
print-%: ; @echo '$(subst ','\'',$*=$($*))'


==> tab/submodule/2021-gecco-conduit/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> tab/submodule/2021-gecco-conduit/fig/asynchronicity_modes.tex <==
\begin{table}
  \begin{tabular}{ccl}
    \toprule
    Mode & Description\\
    \midrule
    0 & Barrier sync every update\\
    1 & Rolling barrier sync\\
    2 & Fixed barrier sync\\
    3 & No barrier sync\\
    4 & No inter-cpu communication\\
  \bottomrule
\end{tabular}
  \caption{Asynchronicity modes used for benchmarking experiments, arranged from most to least synchronized.}
  \label{tab:asynchronicity_modes}
\end{table}


==> tab/submodule/2021-gecco-conduit/fig/conduit.tex <==
   \begin{figure}[thpb]
      \centering
      \includegraphics[width=0.8\linewidth]{img/conduit}
      \caption{Schematic of Conduit's \texttt{Inlet} and \texttt{Outlet} object scheme.
      Intra-thread, inter-thread, or inter-process communication behavior is performed by an underlying \texttt{Duct} object.
      The underlying communication mechanism used is transparent to the end-user.
      }
      \label{fig:conduit}
   \end{figure}

==> tab/submodule/2021-gecco-conduit/fig/multiprocess_benchmarks.tex <==
\begin{figure}[thpb]
      \centering

    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{chart/multiprocess-graph-coloring}
    \caption{Graph coloring per-process update rate. Higher is better.}
    \label{fig:multiprocess_graph_coloring_update_rate}
    \end{subfigure}

    \begin{subfigure}[b]{0.49\textwidth}
      \centering
      \includegraphics[width=\linewidth]{chart/multiprocess-graph-coloring-solution-quality}
      \caption{Graph coloring solution conflicts. Lower is better.}
      \label{fig:multiprocess_graph_coloring_solution_quality}
    \end{subfigure}

  \begin{subfigure}[b]{0.49\textwidth}
    \centering
  \includegraphics[width=\linewidth]{chart/multiprocess-digital-evolution}
  \caption{Digital evolution per-process update rate. Higher is better.}
  \label{fig:multiprocess_digital_evolution_update_rate}
  \end{subfigure}

  \caption{Multiprocess benchmark results. Bars represent bootstrapped 95\% confidence intervals. }
  \label{fig:multiprocess_benchmarks}
\end{figure}


==> tab/submodule/2021-gecco-conduit/fig/multithread_benchmarks.tex <==
  \begin{figure}[thpb]
      \centering
    \begin{subfigure}[b]{0.49\textwidth}
      \centering
      \includegraphics[width=\linewidth]{chart/multithread-graph-coloring}
     \caption{Graph coloring per-thread update rate. Higher is better.}
         \label{fig:multithread_graph_coloring_update_rate}
      \end{subfigure}

    \begin{subfigure}[b]{0.49\textwidth}
      \centering
      \includegraphics[width=\linewidth]{chart/multithread-graph-coloring-solution-quality}
      \caption{Graph coloring solution conflicts. Lower is better.}
         \label{fig:multithread_graph_coloring_solution_quality}
    \end{subfigure}


    \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\linewidth]{chart/multithread-digital-evolution}
    \caption{Digital evolution per-thread update rate. Higher is better.}
         \label{fig:multithread_digital_evolution_update_rate}
    \end{subfigure}

    \caption{Multithread benchmark results. Bars represent bootstrapped 95\% confidence intervals. }
      \label{fig:multithread_benchmarks}
  \end{figure}


==> tab/submodule/2021-gecco-conduit/tex/abstract.tex <==
\begin{abstract}
% Developing software to effectively take advantage of growth in parallel and distributed processing capacity poses significant challenges.
% Best-effort computing models have been proposed as a strategy to overcome challenges around harnessing high performance computing at extreme scale.
% These models relax synchronization and hardware reliability requirements, accepting nondeterminism in exchange for efficiency.
% This trade-off, inherent to best-effort computing, is often compatible with nature-inspired computing methods.
% Although many programming languages and frameworks aim to facilitate software development for high performance applications, existing tools do not directly provide a prepackaged best-effort interface.
% The Conduit C++ Library aims to provide a convenient interface for best-effort inter-thread and inter-process communication.
% Here, we describe the motivation, objectives, design, and implementation of the library.
% Benchmarks on a communication-intensive graph coloring problem and a compute-intensive digital evolution simulation, show that Conduit's best-effort model can improve scaling efficiency and solution quality, particularly in a distributed, multi-node context.

% Conduit will be useful facilitated efficient, scalable parallel and distributed implementations of natural computing algorithms.

Developing software to effectively take advantage of growth in parallel and distributed processing capacity poses significant challenges.
Traditional programming techniques allow a user to assume that execution, message passing, and memory are always kept synchronized.
However, maintaining this consistency becomes increasingly costly at scale. 
One proposed strategy is ``best-effort computing'', which relaxes synchronization and hardware reliability requirements, accepting nondeterminism in exchange for efficiency.
Although many programming languages and frameworks aim to facilitate software development for high performance applications, existing tools do not directly provide a prepackaged best-effort interface.
The Conduit C++ Library aims to provide such an interface for convenient implementation of software that uses best-effort inter-thread and inter-process communication.
Here, we describe the motivation, objectives, design, and implementation of the library.
Benchmarks on a communication-intensive graph coloring problem and a compute-intensive digital evolution simulation show that Conduit's best-effort model can improve scaling efficiency and solution quality, particularly in a distributed, multi-node context.
%% Conduit will be useful facilitated efficient, scalable parallel and distributed implementations of natural computing algorithms. (this is why you care as a GP person)

\end{abstract}




==> tab/submodule/2021-gecco-conduit/tex/acknowledgements.tex <==
\begin{acks}
\footnotesize
This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.

\end{acks}

==> tab/submodule/2021-gecco-conduit/tex/conclusion.tex <==
\section{Conclusion}

Benchmarks show that best-effort communication through Conduit enables significantly better computational performance under high thread and process counts.
We also demonstrated how, in the case of the graph coloring benchmark, best-effort communication can help achieve tangibly better solution quality within a fixed time constraint, as well.  
We observed the greatest relative speedup under distributed communciation-heavy workloads --- about $7.8\times$ on the graph coloring benchmark.
Distributing the computation-heavy digital evolution benchmark workload across independent nodes yielded the strongest scaling of our benchmarks, achieving at 64 processes 92\% the update-rate of single-process execution. 

In future work, we plan to further characterize the performance of the Conduit's best-effort model with respect to the digital evolution simulation, looking directly at quality of service metrics such as message latency and frequency of dropped messages.
We are also eager to investigate how Conduit's best-effort communication model scales on much larger process counts, perhaps on the order of hundreds or thousands of cores.

Development of the Conduit library stemmed from a practical need for an abstract, prepackaged interface to support our digital evolution research.
We hope that making this library available to the community can reduce domain expertise and programmability barriers to taking advantage of the best-effort communication model to efficiently leverage burgeoning parallel and distributed computing power. 

==> tab/submodule/2021-gecco-conduit/tex/design.tex <==
\section{Library Design}

\input{fig/conduit.tex}

The Conduit C++ Library aims to compliment the parallel and distributed programming ecosystem by providing an abstracted best-effort interface to application programmers.
Under Conduit's interface, more recent messages may preempt existing ones, messages may be dropped under backlog conditions, and read operations may opt to view the most recently received message in lieu of waiting for an expected message.

Conduit represents communication in terms of a paired \texttt{Inlet}, which accepts messages, and \texttt{Outlet}, which dispenses messages.
An \texttt{Inlet} and \texttt{Outlet} may exchange messages via an intra-thread, inter-thread, or inter-process communication procedure, depending on the runtime state of an underlying \texttt{Duct} object.
Figure \ref{fig:conduit} provides a schematic overview.
The implementation of intra-thread, inter-thread, and inter-process communication procedures may be configured at compile-time.
Conduit provides a library of intra-thread, inter-thread, and inter-process implementations to choose from and allows end-users to build their own.

The \texttt{Inlet} provides a non-blocking \texttt{TryPut()} method, which attempts to queue a message for its corresponding \texttt{Outlet} but may drop it under backlog conditions, as well as a \texttt{Put()} method, which block under backlog conditions until buffer space is available to queue the message is available.
The \texttt{Outlet} provides a \texttt{TryStep()} and \texttt{Jump()} methods to load the next or latest message, respectively.
If no new messages are available, the last-received message will be accessed.
The \texttt{Outlet} also provides a \texttt{Step()} method, which will block until a new message is received.
At run time, \texttt{Duct}s can be created or modified to perform intrathread, interthread, or interprocess communication. 

In addition to this granular connection-level interface, Conduit provides a network-level interface where the user defines their computation in terms of a directed graph.
In this network topology, nodes represent simulation elements and edges represent communication channels.
The library will assign nodes in that topology to available threads across available processes and automatically instantiate appropriate conduits.
Individual threads of execution can then launch and freely process computational updates on their assigned nodes while receiving messages from nodes assigned to other processes as they become available.
Conduit provides several pre-defined standard topologies and node-assignment algorithms.
However, users can also opt to use the NetworkX graph library \cite{hagberg2008exploring} to generate arbitrary topologies and the METIS software package \cite{gupta1997fast} to automatically balance expected load across available threads and processes while minimizing inter-process and inter-thread communication.

Defining program logic in terms of atomic, inter-communicating simulation elements provides significant programmability advantages.
Such code can be written in terms of interactions between intuitive domain-specific objects (e.g., digital organisms that interact with one another, subpopulations with migration, etc.), while leaving the task of mapping onto hardware resources to automatic management by the underlying framework.
However, a naive implementation of this approach would entail significant inefficiency, particularly with inter-process communication which has a large overhead.
Imagine, for example, a processes dispatching independent MPI calls for each communication channel between another process and the thousands of atomic simulation elements it holds.
Conduit addresses this issue by providing duct implementations that automatically consolidate messages between processes into single MPI calls.
These implementations support a ``pooling'' mechanism, in which a consolidated MPI call is dispatched once each constituent \texttt{Inlet} has received a single message, and a ``aggregation'' mechanism, in which arbitrary numbers of messages can be contributed from each \texttt{Inlet}.

Conduit is made freely available under a MIT License as a header-only C++17 software package at \url{https://github.com/mmore500/conduit}.
Conduit was built using the cereal C++11 Library for serialization \cite{voorhies2017cereal} and the Empirical C++ Library \cite{charles_ofria_2019_2575607}.


==> tab/submodule/2021-gecco-conduit/tex/implementation.tex <==
\section{ Implementation }

Conduit's implementation has been developed around the following principles.

\begin{itemize}
    \item \textbf{overdecomposition}: Conduit provides a uniform API for intra-thread, inter-thread, and inter-process communication between agents.
    \item \textbf{testability}: Interchangeablility of inter-thread and inter-process communication for intra-thread communication makes software more readily unit-testable.
    \item \textbf{don't use what you don't want}: Multi-thread execution may be performed without MPI runtime.
    \item \textbf{don't pay for what you don't use}: Intra-thread, inter-thread, and inter-process communication are explicitly handled by separate, optimized implementations. 
    \item \textbf{modularity}: Different intra-thread, inter-thread, or inter-process implementations can be trivially interchanged for rapid prototyping and tuning.
    \item \textbf{flexibility}: Communication primitives may trivially rearranged to form arbitrary network structures. 
    \item \textbf{extensibility}: Users may provide communication implementations or network topologies.
    \item \textbf{lightweight}: The core components of Conduit are built as a header-only library.
    \item \textbf{portability}: Conduit is built using MPI and C++17 standards.
    \item \textbf{interoperability}: Conduit is compatible with other multithread and MPI code.
    \item \textbf{simplicity}: Conduit manages resource initialization and lifetime automatically.
    % \item \textbf{intuitiveness}: TODO object-oriented model with a simple API and an intuitive real-world analogy.
\end{itemize}

Source code is hosted on GitHub at \url{https://github.com/mmore500/conduit}, made freely available under a MIT License.
Documentation is hosted on ReadTheDocs at \url{https://conduit.fyi}.
A containerized build environment for Conduit is hosted on DockerHub at \url{https://hub.docker.com/r/mmore500/conduit}.

==> tab/submodule/2021-gecco-conduit/tex/introduction.tex <==
\section{Introduction}

The parallel and distributed processing capacity of high-performance computing clusters continues to grow rapidly and enable profound scientific and industrial innovations \cite{gagliardi2019international}.    
Hardware advances afford great opportunity, but also pose a serious challenge: developing approaches to effectively harness it.
As HPC systems scale, deterministic algorithms depending on global synchronization become increasingly costly \cite{gropp2013programming,dongarra2014applied}.

Best-effort computing, where data dependencies are relaxed to reduce synchronization \cite{chakradhar2010best}, can improve scalability \cite{meng2009best}.
Evolutionary algorithms typically perform perform a search or optimization with many acceptable results using pseudo-stochastic methods.
Algorithms with these properties can often tolerate significant perturbations, including relaxation of synchronization requirements in the underlying algorithm.
For example, island model genetic algorithms have been shown to perform well with asynchronous migration \cite{izzo2009parallel}.
While not the focus of this paper, the original interest that motivated development of the Conduit library stems from work exploring open-ended evolution.
Researchers in this domain study long-term dynamics of evolutionary systems in order to understand factors that affect these systems' potential to generate ongoing novelty \cite{taylor2016open}.
Some recent evidence suggests that the generative potential of systems devised to study open-ended evolution is --- at least in part --- meaningfully constrained by available compute resources \cite{channon2019maximum}.
Such observations raise the question of how to design parallel and distributed open-ended evolution systems.

The concept of indefinite scalability was developed to describe constraints distributed systems would face at the asymptote of technological (and even physical) constraints.
Indefinite scalability theory posits that such systems would necessitate
\begin{itemize}
    \item asynchronous operation,
    \item decentralized networking,
    \item interchangeable components (i.e., no global identifiers),
    \item and graceful degradation under hardware failure \cite{ackley2011pursue}.
\end{itemize}
Although bespoke experimental hardware such as Illuminato X machina has been developed to demonstrate aspects of the indefinite scalability paradigm \cite{ackley2011homeostatic}, practical contemporary work scaling up evolving systems necessitates working with commercially-available hardware.
However, existing distributed computing frameworks for contemporary high-performance computing hardware do not explicitly expose a convenient best-effort interface.
In our current work, we focus on asynchronous operation and decentralization.
We leave system robustness and resistance to hardware degradation to future work.

The Message Passing Interface (MPI) standard \cite{gropp1996high} represents the mainstay for high-performance computing applications.
This standard exposes communication primitives directly to the end user.
MPI's nonblocking communication primitives, in particular, are sufficient to program distributed computations with relaxed synchronization requirements.
Although its explicit, imperative nature enables precise control over execution, it also poses significant expense in terms of programability.
This cost manifests in terms of programmer productivity, domain knowledge requirements, software quality, and difficulty tuning for performance due to program brittleness \cite{gu2019comparative, tang2014mpi}.

In response to programmability concerns, many frameworks have arisen to offer useful parallel and distributed programming abstractions.
Task-based frameworks such as Charm++ \cite{kale1993charm++}, Legion \cite{bauer2012legion}, Cilk \cite{blumofe1996cilk}, and Threading Building Blocks (TBB) \cite{reinders2007intel} describe the dependency relationships among computational tasks and associated data and relies on an associated runtime to automatically schedule and manage execution.
These frameworks assume a deterministic relationship between tasks.
In a similar vein, programming languages and extensions like Unified Parallel C (UPC) \cite{el2006upc} and Chapel \cite{chamberlain2007parallel} rely on programmers to direct execution, but equips them with powerful abstractions, such as global shared memory.
However, Chapel's memory model explicitly forbids data races and UPC ultimately relies on a barrier model for data transfer.

==> tab/submodule/2021-gecco-conduit/tex/methods.tex <==
\section{Methods}

We performed two benchmarks to compare the performance of Conduit's best-effort approach to a traditional synchronous model.
We tested our benchmarks across both a multithread, shared-memory context and a distributed, multinode context.
In each hardware context, we assessed performance on two algorithmic contexts: a communication-intensive distributed graph coloring problem (Section \ref{sec:graph_coloring_benchmark}) and a compute-intensive digital evolution simulation (Section \ref{sec:digital_evolution_benchmark}).
The latter benchmark --- presented in Section \ref{sec:digital_evolution_benchmark} --- grew out of the original work developing the Conduit library to support large-scale experimental systems to study open-ended evolution.
The former benchmark --- presented in Section \ref{sec:graph_coloring_benchmark} --- complements the first by providing a clear definition of solution quality.
Metrics to define solution quality in the open-ended digital evolution context remain a topic of active research.

\subsection{ Graph Coloring Benchmark } \label{sec:graph_coloring_benchmark}

The graph coloring benchmark employs a graph coloring algorithm designed for distributed WLAN channel selection \cite{leith2012wlan}.
In this algorithm, nodes begin by randomly choosing a color.
Each computational update, nodes test for any neighbor with the same color.
If and only if a conflicting neighbor is detected, nodes randomly select another color.
The probability of selecting each possible color is stored in array associated with each node.
Before selecting a new color, the stored probability of selecting the current (conflicting) color is decreased by a multiplicative factor $b$.
We used $b=0.1$, as suggested by Leith et al.
Likewise, the stored probability of selecting all others is increased by a multiplicative factor.
Regardless of whether their color changed, nodes transmit their current color to their neighbor.

Our benchmarks focus on weak scalability, using a fixed problem size of 2048 graph nodes per thread or process.
These nodes were arranged in a two-dimensional grid topology where each node had three possible colors and four neighbors.
We implement the algorithm with a single Conduit communication layer carrying graph color as an unsigned integer.
We used Conduit's built-in pooling feature to consolidate color information into a single MPI message between pairs of communicating processes each update. 
We performed five replicates, each with a five second simulation runtime.
Solution error was measured as the number of graph color conflicts remaining at the end of the benchmark. 

\subsection{ Digital Evolution Benchmark } \label{sec:digital_evolution_benchmark}

The digital evolution benchmark runs the DISHTINY (DIStributed Hierarchical Transitions in Individuality) artificial life framework.
This system is designed to study major transitions in evolution, events where lower-level organisms unite to form a self-replicating entity.
The evolution of multicellularity and eusociality exemplify such transitions. 
Previous work with DISHTINY has explored methods for selecting traits characteristic of multicellularity such as reproductive division of labor, resource sharing within kin groups, resource investment in offspring, and adaptive apoptosis \cite{moreno2019toward}.

DISHTINY simulates a fixed-size toroidal grid populated by digital cells.
Cells can sense attributes of their immediate neighbors, can communicate with those neighbors through arbitrary message passing, and can interact with neighboring cells cooperatively through resource sharing or competitively through antagonistic competition to spawn daughter cells into limited space.
This cell behavior is controlled by SignalGP event-driven linear genetic programs \cite{lalejini2018evolving}.
Full details of the DISHTINY simulation are available in \cite{moreno2021exploring}.

We use Conduit-based messaging channels to manage all interactions between neighboring cells.
During a computational update, each cell advances its internal state and pushes information about its current state to neighbor cells.
Several independent messaging layers handle disparate aspects of cell-cell interaction, including
\begin{itemize}
  \item Cell spawn messages, which contain arbitrary-length genomes (seeded at 100 12-byte instructions with a hard cap of 1000 instructions). These are handled every 16 updates and use Conduit's built-in aggregation support for inter-process transfer.
  \item Resource transfer messages, consisting of a 4-byte float value. These are handled every update and use Conduit's built-in pooling support for inter-process transfer.
  \item Cell-cell communication messages, consisting of arbitrarily many 20-byte packets dispatched by genetic program execution. These are handled every 16 updates and use Conduit's built-in aggregation support for inter-process transfer.
  \item Environmental state messages, consisting of a 216-byte struct of data. These are handled every 8 updates and use conduit's built-in pooling support for inter-process transfer.
  \item Multicellular kin-group size detection messages, consisting of a 16-byte bitstring. These are handled every update and use Conduit's built-in pooling support for inter-process transfer.
\end{itemize}

Implementing all cell-cell interaction via Conduit-based messaging channels allows the simulation to be parallelized down to the granularity, potentially, of individual cells.
However, in practice, for this benchmarking we assign 3600 cells to each thread or process.
Because all cell-cell interactions occur via Conduit-based messaging channels, logically-neighboring cells can interact fully whether or not they are located on the same thread or process (albeit with potential irregularities due to best-effort limitations). 
An alternate approach to evolving large populations might be an island model, where Conduit-based messaging channels would be used solely to exchange genomes between otherwise independent populations \cite{bennett1999building}.
However, we chose to instead parallelize DISHTINY as a unified spatial realm in order to enable parent-offspring interaction and leave the door open for future work with multicells that exceed the scope of an individual thread or process.

\subsection{Asynchronicity Modes} \label{sec:asynchronicity_modes}

\input{fig/asynchronicity_modes.tex}

For both benchmarks, we compared performance across a spectrum of synchronization setting, which we term ``asynchronicity modes'' (Table \ref{tab:asynchronicity_modes}).
Asynchronicity mode 0 represents traditional fully-synchronous methodology.
Under this treatment, full barrier synchronization was performed between each computational update.
Asynchronicity mode 3 represents fully asynchronous methodology.
Under this treatment, individual threads or processes performed computational updates freely, incorporating input from other threads or processes on a fully best-effort basis.  

During early development of the library, we discovered that unprocessed messages building up faster than they could be processed --- even if they were being skipped over to only get the latest message --- could degrade quality of service or even cause runtime instability.
We opted for MPI communication primitives that could consume many backlogged messages per call and increased buffer size to address these issues, but remained interested in the possibility of partial synchronization to clear potential message backlogs.
So, we included two partially-synchronized treatments: asynchronicity modes 1 and 2.

In asynchronicity mode 1, threads and processes alternated between performing computational updates for a fixed-time duration and executing a global barrier synchronization.
For the graph coloring benchmark, work was performed in 10ms chunks.
For the digital evolution benchmark, which is more computationally intensive, work was performed in 100ms chunks.
In asynchronicity mode 2, threads and processes executed global barrier synchronizations at predetermined time points.
In both experiments, global barrier synchronization occurred on each time a second of epoch time elapsed.

Finally, asynchronicity mode 4 disables all inter-thread and inter-process communication, including barrier synchronization.
We included this mode to isolate the impact on performance of communication between threads and processes from other factors potentially affecting performance, such as cache crowding.
In this run mode for the graph coloring benchmark, all calls to put messages into or pull messages out of ducts between processes or threads were skipped (except after the benchmark concluded, when assessing solution quality).
Because of its larger footprint, incorporating logic into the digital evolution simulation to disable all inter-thread and inter-process messaging was impractical.
Instead, we launched multiple instances of the simulation as fully-independent processes and measured performance of each.

\subsection{Code, Data, and Reproducibility}

Benchmarking experiments were performed on [redacted for double-blind review]'s High Performance Computing Center, a cluster of hundreds of heterogeneous x86 nodes linked with InfiniBand interconnects.
For multithread experiments, benchmarks for each thread count were collected from the same node.
For multiprocess experiments, each processes was assigned to a distinct node in order to ensure results were representative of performance in a distributed context.
All multiprocess benchmarks recorded from the same collection of nodes.
Hostnames are recorded for each benchmark data point.
For an exact accounting of hardware architectures used, these hostnames can be crossreferenced with a table included with the data that summarizes the cluster's node configurations.

Code for the distributed graph coloring benchmark is available at \url{https://github.com/mmore500/conduit} under \\ \texttt{demos/channel\_selection}.
Code for the digital evolution simulation benchmark is available at \url{https://github.com/mmore500/dishtiny}.
Exact versions of software used are recorded with each benchmark data point.
Data is available via the Open Science Framework at \url{https://osf.io/7jkgp/} \cite{foster2017open}.
An in-browser notebook for all reported statistics and data visualizations and is available via Binder at \url{https://mybinder.org/v2/gh/mmore500/conduit/HEAD?filepath=binder\%2F} \cite{jupyter2018binder}.

==> tab/submodule/2021-gecco-conduit/tex/results.tex <==
\section{Results and Discussion}

\subsection{Multithread Benchmarks}

\input{fig/multithread_benchmarks.tex}

Figure \ref{fig:multithread_graph_coloring_update_rate} presents per-cpu algorithm update rate for the graph coloring benchmark at 1, 4, 16, and 64 threads.
Update rate performance decreased with increasing multithreading across all asynchronicity modes.
This performance degradation was rather severe --- per-cpu update rate decreased by 61\% between 1 and 4 threads and by about another 75\% between 4 and 64 threads.
Surprisingly, this issue appears largely unrelated to inter-thread communication, as it was also observed in asynchronicity mode 4, where all interthread communication is disabled.
Perhaps per-cpu update rate degradation under threading was induced by strain on a limited system resource like memory cache or access to the system clock (which was used to control run timing).
This unexpectedly severe phenomenon merits further investigation to fully in future work with this benchmark.

Nevertheless, we were able to observe significantly better performance of best-effort asynchronicity modes 1, 2, and 3 at high thread counts. 
At 64 threads, these run modes significantly outperformed the fully-synchronized mode 0 ($p < 0.05$, non-overlapping 95\% confidence intervals).
Likewise, as shown in Figure \ref{fig:multithread_graph_coloring_solution_quality}, best-effort asynchronicity modes were able to deliver significantly better graph coloring solutions within the allotted compute time than the fully-synchronized mode 0 ($p < 0.05$, non-overlapping 95\% confidence intervals).

Figure \ref{fig:multithread_digital_evolution_update_rate} shows per-cpu algorithm update rate for the digital evolution benchmark at 1, 4, 16, and 64 threads.
Similarly to the graph coloring benchmark, update rate performance decreased with increasing multithreading across all asynchronicity modes --- including mode 4, which eschews inter-thread communication.
Even without communication between threads, with 64 threads each thread performed updates at only 61\% the rate of a lone thread.
At 64 threads, best-effort asynchronicity modes 1, 2, and 3 exhibit about 43\% the update-rate performance of a lone thread.
Although best-effort inter-thread communication only exhibits half the update-rate performance of completely decoupled execution at 64 threads, this update-rate performance is roughly $2.1\times$ that of the fully-synchronous mode 0.
Indeed, best-effort modes significantly outperform the fully-synchronous mode on the digital evolution benchmark at both 16 and 64 threads ($p < 0.05$, non-overlapping 95\% confidence intervals).

\subsection{Multiprocess Benchmarks}

\input{fig/multiprocess_benchmarks.tex}

Figure \ref{fig:multiprocess_graph_coloring_update_rate} shows per-cpu algorithm update rate for the graph coloring benchmark at 1, 4, 16, and 64 processes.
Unlike the multithreaded benchmark, multiprocess graph coloring exhibits consistent update-rate performance across process counts under asynchronicity mode 4, where inter-thread communication is disabled.
This matches the expectation that, indeed, with comparable hardware a single process should exhibit the same mean performance as any number of completely decoupled processes.
At 64 processes, best-effort asynchronicity mode 3 exhibits about 63\% the update-rate performance of single-process execution. 
This represents about an $7.8\times$ speedup compared to fully-synchronous mode 0.
Indeed, best-effort mode 3 enables significantly better per-cpu update rates at 4, 16, and 64 processes ($p < 0.05$, non-overlapping 95\% confidence intervals).

Likewise, shown in Figure \ref{fig:multiprocess_graph_coloring_solution_quality}, best-effort asynchronicity mode 3 yields significantly better graph-coloring results within the allotted time at 4, 16, and 64 processes ($p < 0.05$, non-overlapping 95\% confidence intervals).
Interestingly, partial-synchronization modes 1 and 2 exhibited highly inconsistent solution quality performance at 16 and 64 process count benchmarks.
Fixed-timepoint barrier sync (mode 2) had particularly poor performance performance at 64 processes (note the log-scale axis).
We suspect this was caused by a race condition where workers would assign sync points to different fixed points different based on slightly different startup times (i.e., process 0 syncs at seconds 0, 1, 2... while process 1 syncs at seconds 1, 2, 3..).

Figure \ref{fig:multiprocess_digital_evolution_update_rate} presents per-cpu algorithm update rate for the digital evolution benchmark at 1, 4, 16, and 64 processes.
Relative performance fares well at high process counts under this relatively computation-heavy workload, with 64-process fully best-effort simulation exhibiting about 92\% the update rate of single-process simulation.
This represents a $2.1\times$ speedup compared to the fully-synchronous run mode 0.
Best-effort significantly mode 3 outperforms the per-cpu update rate of fully-synchronous mode 0 at process counts 16 and 64 ($p < 0.05$, non-overlapping 95\% confidence intervals).


==> tab/submodule/conduit-binder/Dockerfile <==
# Pull base image.
FROM ubuntu:bionic-20180125@sha256:d6f6cc62b6bed64387d84ca227b76b9cc45049b0d0aefee0deec21ed19a300bf

COPY . /opt/conduit/

SHELL ["/bin/bash", "-c"]

# Define default working directory.
WORKDIR /opt/conduit

# Prevent interactive time zone config.
# adapted from https://askubuntu.com/a/1013396
ENV DEBIAN_FRONTEND=noninteractive

# adapted from https://users.open-mpi.narkive.com/tEPxZF0B/ompi-users-how-to-get-rid-of-openmpi-warning-unable-to-find-any-relevant-network-interfaces
# see also https://github.com/open-mpi/ompi-www/issues/161#issue-390004007
RUN \
  mkdir -p "/root/.openmpi" \
    && \
  mkdir -p "/home/user/.openmpi" \
    && \
  echo "btl_base_warn_component_unused = 0" >> /etc/openmpi-mca-params.conf \
    && \
  echo "btl_base_warn_component_unused = 0" >> /root/.openmpi/mca-params.conf \
    && \
  echo "btl_base_warn_component_unused = 0" >> /home/user/.openmpi/mca-params.conf \
    && \
  echo "configured system-wide openmpi mca parameters"

RUN \
  echo 'Acquire::http::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::ftp::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::Retries "100";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo "buffed apt-get resiliency"

RUN \
  find /etc/apt -type f -name '*.list' -exec sed -i 's/\(^deb.*-backports.*\)/#\1/; s/\(^deb.*-updates.*\)/#\1/; s/\(^deb.*-proposed.*\)/#\1/; s/\(^deb.*-security.*\)/#\1/' {} + \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "removed -backports, -updates, -proposed, -security repositories"

RUN \
  apt-get update -qq \
    && \
  apt-get install -y --allow-downgrades --no-install-recommends \
    build-essential \
    ca-certificates \
    cmake \
    curl \
    doxygen \
    emacs \
    fonts-liberation \
    gconf-service \
    gdb \
    gpg-agent \
    gzip \
    hdf5-helpers \
    hdf5-tools \
    htop \
    libappindicator1 \
    libasound2 \
    libatk1.0-0 \
    libc6 \
    libcairo2 \
    libcups2 \
    libcurl4 \
    libcurl4-openssl-dev \
    libdbus-1-3 \
    libexpat1 \
    libfontconfig1 \
    libgconf-2-4 \
    libgdk-pixbuf2.0-0 \
    libglib2.0-0 \
    libgtk-3-0 \
    libhdf5-100 \
    libhdf5-cpp-100 \
    libhdf5-dev \
    libhdf5-doc \
    libhdf5-mpi-dev \
    libhdf5-mpich-100 \
    libhdf5-mpich-dev \
    libhdf5-openmpi-100 \
    libhdf5-openmpi-dev \
    libhdf5-serial-dev \
    libmpich-dev \
    libmpich12 \
    libnspr4 \
    libnss3 \
    libopenmpi-dev \
    libopenmpi2 \
    libpango-1.0-0 \
    libpangocairo-1.0-0 \
    libpthread-stubs0-dev \
    libstdc++-7-dev \
    libstdc++6=8-20180414-1ubuntu2 \
    libx11-6 \
    libx11-xcb1 \
    libxcb1 \
    libxcomposite1 \
    libxcursor1 \
    libxdamage1 \
    libxext6 \
    libxfixes3 \
    libxi6 \
    libxrandr2 \
    libxrender1 \
    libxss1 \
    libxtst6 \
    locales \
    lsb-release \
    man \
    mpich \
    multitail \
    nano \
    ninja-build \
    nodejs \
    npm \
    openmpi-bin \
    openmpi-common \
    openmpi-doc \
    openssh-server \
    python-dev \
    python-h5py \
    python-pip \
    python-setuptools \
    python-sphinx \
    python-virtualenv \
    python-wheel \
    python3-dev \
    python3-h5py \
    python3-pip \
    python3-setuptools \
    python3-sphinx \
    python3-virtualenv \
    python3-wheel \
    rsync \
    slurm-client \
    software-properties-common \
    tar \
    unzip \
    vim \
    wget \
    xdg-utils \
    && \
  add-apt-repository ppa:git-core/ppa -y \
    && \
  apt-get update -qq \
    && \
  apt-get install -y --no-install-recommends git \
    && \
  apt-get clean \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "installed fundamentals"

# adapted in part from https://askubuntu.com/a/916451
RUN \
  apt-get update -qq \
    && \
  rm /etc/apt/apt.conf.d/docker-gzip-indexes \
    && \
  apt-get purge apt-show-versions \
    && \
  rm /var/lib/apt/lists/*lz4 \
    && \
  apt-get -o Acquire::GzipIndexes=false update \
    && \
  add-apt-repository -y ppa:ubuntu-toolchain-r/test \
    && \
  wget -O - https://apt.llvm.org/llvm-snapshot.gpg.key | apt-key add - \
    && \
  apt-add-repository "deb https://apt.llvm.org/xenial/ llvm-toolchain-xenial-7 main" \
    && \
  add-apt-repository -y ppa:ubuntu-toolchain-r/test \
    && \
  apt-get update -qq \
    && \
  apt-get clean \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "configured packaging system"

RUN \
  apt-get update -qq \
    && \
  apt-get install -qq \
    libclang-7-dev=1:7.1.0~svn353565-1~exp1~20190408084827.60 \
    llvm-7=1:7.1.0~svn353565-1~exp1~20190408084827.60 \
    llvm-7-dev=1:7.1.0~svn353565-1~exp1~20190408084827.60 \
    clang-7=1:7.1.0~svn353565-1~exp1~20190408084827.60 \
    g++-9=9.4.0-1ubuntu1~18.04 \
    && \
  apt-get clean \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "installed llvm-7 dependencies"

# magic from https://github.com/puppeteer/puppeteer/issues/3451#issuecomment-523961368
RUN echo 'kernel.unprivileged_userns_clone=1' > /etc/sysctl.d/userns.conf

RUN \
  pip3 install  --timeout 60 --retries 100 -r /opt/conduit/third-party/requirements.txt \
    && \
  pip3 install  --timeout 60 --retries 100 -r /opt/conduit/docs/requirements.txt \
    && \
  echo "installed Python packages"

RUN \
  update-alternatives --install /usr/bin/g++ g++ /usr/bin/g++-9 90 \
    && \
  update-alternatives --install /usr/bin/clang++ clang++ /usr/bin/clang++-7 90 \
    && \
  update-alternatives --install /usr/bin/llvm-config llvm-config /usr/bin/llvm-config-7 90 \
    && \
  update-alternatives --install /usr/bin/llvm-profdata llvm-profdata /usr/bin/llvm-profdata-7 90 \
    && \
  update-alternatives --install /usr/bin/llvm-cov llvm-cov /usr/bin/llvm-cov-7 90 \
    && \
  npm install -g n@6.7.0 \
    && \
  n 12.18.2 \
    && \
  export python="/usr/bin/python" \
    && \
  npm install source-map@0.7.3 \
    && \
  echo "finalized dependency versions"

RUN \
  npm install -g jsonlint@1.6.3 \
    && \
  echo "installed npm dependencies"

RUN \
  cd third-party \
    && \
  ./install_dependencies.sh \
    && \
  echo "installed third party dependencies"

# set up locale
# adapted from https://stackoverflow.com/a/55077451
RUN \
  locale-gen en_US.UTF-8 \
    && \
  echo "generated en_US.UTF-8 locale"

# Set enviroment variables
# Use mimalloc override within the container.
ENV LD_PRELOAD=/usr/local/lib/mimalloc-1.6/libmimalloc.so
ENV LC_ALL=C.UTF-8
ENV LANG=C.UTF-8

RUN \
  git remote set-url origin https://github.com/mmore500/conduit.git \
    && \
  echo "switched to https origin remote url"

# Perform any further action as an unprivileged user.
# adapted from https://stackoverflow.com/a/27703359
# and https://superuser.com/a/235398
RUN \
  useradd --create-home --shell /bin/bash user \
    && \
  groupadd group \
    && \
  gpasswd -a user group \
    && \
  chgrp --recursive user /opt \
    && \
  chmod --recursive g+rwx /opt \
    && \
  chmod --recursive g+rwx /home/user \
    && \
  chown -R user /home/user/ \
    && \
  echo "user added and granted permissions to /opt and /home/user"

RUN \
  mkdir /context/ \
    && \
  chown user:user /context/ \
    && \
  mkdir /__w/ \
    && \
  chown user:user /__w/ \
    && \
  echo "/context/ /__w/ directories set up, user granted permissions"

USER user

CMD ["bash"]


==> tab/submodule/conduit-binder/Makefile <==
SHELL := /bin/bash

# Project-specific settings
PROJECT := conduit
EMP_DIR := third-party/Empirical/include/emp

# Flags to use regardless of compiler
CFLAGS_all := -pipe -Wall -Wno-unused-function -std=c++17 -Iinclude/ -fopenmp

# Native compiler information
CFLAGS_nat := -O3 -DNDEBUG -O3 -flto -march=native $(CFLAGS_all)
CFLAGS_nat_debug := -g $(CFLAGS_all)
UIT_MPICXX ?= mpicxx
UIT_MPIEXEC ?= mpiexec

# Emscripten compiler information
CXX_web := emcc
OFLAGS_web_all := -s "EXTRA_EXPORTED_RUNTIME_METHODS=['ccall', 'cwrap']" -s TOTAL_MEMORY=67108864 --js-library $(EMP_DIR)/web/library_emp.js -s EXPORTED_FUNCTIONS="['_main', '_empCppCallback', '_empDoCppCallback']" -s DISABLE_EXCEPTION_CATCHING=1 -s NO_EXIT_RUNTIME=1 #--embed-file configs
OFLAGS_web := -Oz -DNDEBUG
OFLAGS_web_debug := -g4 -Oz -Wno-dollar-in-identifier-extension

CFLAGS_web := $(CFLAGS_all) $(OFLAGS_web) $(OFLAGS_web_all)
CFLAGS_web_debug := $(CFLAGS_all) $(OFLAGS_web_debug) $(OFLAGS_web_all)


default: $(PROJECT)
native: $(PROJECT)
web: $(PROJECT).js documentation-coverage-badge.json version-badge.json doto-badge.json

omp: CFLAGS_nat := $(CFLAGS_nat) -fopenmp
omp: $(PROJECT)

debug: CFLAGS_nat := $(CFLAGS_nat_debug)
debug: $(PROJECT)

debug-web: CFLAGS_web := $(CFLAGS_web_debug)
debug-web: $(PROJECT).js

web-debug: debug-web

$(PROJECT): source/native/$(PROJECT).cpp
	$(UIT_MPICXX) $(CFLAGS_nat) source/native/$(PROJECT).cpp -lstdc++fs -lbenchmark -lmetis -lpthread -o $(PROJECT)
	@echo To build the web version use: make web

$(PROJECT).js: source/web/$(PROJECT)-web.cpp
	source third-party/emsdk/emsdk_env.sh; \
	$(CXX_web) $(CFLAGS_web) source/web/$(PROJECT)-web.cpp -o web/$(PROJECT).js

serve:
	python3 -m http.server

install-coverage-dependencies:
	git submodule init && git submodule update \
		&& cd third-party/force-cover && make

cov: install-coverage-dependencies
	cd tests && make cov

documentation-coverage:
	cd docs && make coverage

documentation-coverage-badge.json: documentation-coverage
	python3 ci/parse_documentation_coverage.py docs/_build/doc-coverage.json > web/documentation-coverage-badge.json

version-badge.json:
	python3 ci/parse_version.py .bumpversion.cfg > web/version-badge.json

doto-badge.json:
	python3 ci/parse_dotos.py $$(./ci/grep_dotos.sh) > web/doto-badge.json

clean:
	rm -f $(PROJECT) web/$(PROJECT).js web/*.js.map web/*.js.map *~ source/*.o web/*.wasm web/*.wast
	rm -rf coverage_include
	cd docs && make clean
	cd demos && make clean
	cd macrobenchmarks && make clean
	cd microbenchmarks && make clean
	cd tests && make clean

docs:
	cd docs && make html

demos:
	cd demos && make

macrobenchmark:
	cd macrobenchmarks && make bench

microbenchmark:
	cd microbenchmarks && make bench

benchmark: macrobenchmark microbenchmark

test-readme-snippets:
	python3 ci/test_readme_snippets.py

test-source: debug debug-web
	$(UIT_MPIEXEC) -n 1 ./conduit | grep -q '>>> end <<<' && echo 'matched!' || exit 1
	npm install
	echo "const puppeteer = require('puppeteer'); var express = require('express'); var app = express(); app.use(express.static('web')); app.listen(3000); express.static.mime.types['wasm'] = 'application/wasm'; function sleep(millis) { return new Promise(resolve => setTimeout(resolve, millis)); } async function run() { const browser = await puppeteer.launch(); const page = await browser.newPage(); await page.goto('http://localhost:3000/conduit.html'); await sleep(1000); const html = await page.content(); console.log(html); browser.close(); process.exit(0); } run();" | node | tr -d '\n' | grep -q "Hello, browser!" && echo "matched!" || exit 1
	echo "const puppeteer = require('puppeteer'); var express = require('express'); var app = express(); app.use(express.static('web')); app.listen(3000); express.static.mime.types['wasm'] = 'application/wasm'; function sleep(millis) { return new Promise(resolve => setTimeout(resolve, millis)); } async function run() { const browser = await puppeteer.launch(); const page = await browser.newPage(); page.on('console', msg => console.log(msg.text())); await page.goto('http://localhost:3000/conduit.html'); await sleep(1000); await page.content(); browser.close(); process.exit(0); } run();" | node | grep -q "Hello, console!" && echo "matched!"|| exit 1

test:
	test $TRAVIS && mkdir -p "~/.openmpi/" && touch "~/.openmpi/mca-params.conf" && grep -qxF 'btl_base_warn_component_used = 0' ~/.openmpi/mca-params.conf || echo 'btl_base_warn_component_used = 0' >> ~/.openmpi/mca-params.conf
	cd tests && make

test-opt:
	test $TRAVIS && mkdir -p "~/.openmpi/" && touch "~/.openmpi/mca-params.conf" && grep -qxF 'btl_base_warn_component_used = 0' ~/.openmpi/mca-params.conf || echo 'btl_base_warn_component_used = 0' >> ~/.openmpi/mca-params.conf
	cd tests && make opt

test-fulldebug:
	test $TRAVIS && mkdir -p "~/.openmpi/" && touch "~/.openmpi/mca-params.conf" && grep -qxF 'btl_base_warn_component_used = 0' ~/.openmpi/mca-params.conf || echo 'btl_base_warn_component_used = 0' >> ~/.openmpi/mca-params.conf
	cd tests && make fulldebug

test-all: test test-opt test-fulldebug

.PHONY: \
	benchmark \
	clean \
	cov \
	demos \
	docs \
	install-coverage-dependencies \
	native \
	macrobenchmark \
	microbenchmark \
	serve \
	test \
	tests \
	web \


# Debugging information
print-%: ; @echo '$(subst ','\'',$*=$($*))'

